Allocation Before Ranking: Decoupled Token Compression for OmniLLMs

Token compression in OmniLLMs is typically posed as a single saliency-ranking problem: score each multimodal token, keep the top-K. We argue this abstraction is mis-specified. The same attention score simultaneously decides two things: how much retained capacity each modality receives, and which tokens within a modality are kept. A shared top-K rule therefore inherits this audio-favoring allocation prior, spending retained capacity on audio before video tokens have a chance to compete. We propose Macer, a training-free compressor that first assigns explicit audio and video budgets, then performs allocation-normalized ranking within each modality at modality-specific shallow layers. Macer significantly reduces token cost while preserving accuracy across audio-grounded, audio--video joint, visual-dominant, and video-centric benchmarks. At 25 % retention, Macer preserves 98.7 % of full-token performance on Qwen2.5-Omni-7B and 97.3 % on Qwen2.5-Omni-3B. On Qwen2.5-Omni-7B, this 25 % setting reaches OmniZip-level performance at 45 % retention while using lower FLOPs. On OmniVinci-9B, the same allocation-before-ranking principle improves over shared top-K ranking by up to 12.9 points.

==> checklist.tex <==
\section*{NeurIPS Paper Checklist}


\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The abstract and introduction state the central claim that shared-ranking compression conflates cross-modal capacity allocation with within-modality token selection, and present \textsc{Macer} as a training-free method that separates these decisions. The scope is limited to the evaluated shared-decoder backbones and benchmarks, with evidence in Sec.~5 and Appendix~F.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A \answerNo{} or \answerNA{} answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{}{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Sec.~6 discusses the scope and limitations of MACER, including its intended model setting and natural directions for future work.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper has no limitation while the answer \answerNo{} means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate ``Limitations'' section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory assumptions and proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper does not present formal theoretical results, theorems, or guarantees. The allocation--selection decomposition is used as an algebraic diagnostic and motivation for the method, with the corresponding equations stated in Sec.~3 and Appendix~C.1.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental result reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Sec.~5.1 specifies the benchmarks, baselines, model backbones, decoding setup, hardware, retention ratios, FLOPs accounting, and fixed deployment defaults. Appendix~A--B provide the evaluation protocol, calibration split, metrics, token statistics, and full \textsc{Macer} procedure.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item If the paper includes experiments, a \answerNo{} answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and\slash or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerNo{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We do not release an open-access public repository at submission time. However, the full \textsc{Macer} procedure is specified in Sec.~4 and Appendix~\ref{app:method_details}, including allocation-normalized modality scoring (Eq.~\ref{eq:appendix_score}), capacity-coordinated splitting (Eqs.~\ref{eq:appendix_budget}--\ref{eq:appendix_capacity}), staged modality-specific pruning (Table~\ref{tab:macer_algorithm}), and the score-aware chunk-coverage greedy rule (Eq.~\ref{eq:appendix_greedy}). All scale-specific calibrated configurations are listed in Table~\ref{tab:macer_defaults}, the evaluation protocol and token statistics are reported in Appendix~\ref{app:protocol}, and the FLOPs accounting is given in Appendix~\ref{app:efficiency}. The experiments use publicly released model backbones (Qwen2.5-Omni-7B/3B and OmniVinci-9B), public benchmarks (AVUTBench, DailyOmni, WorldSense, and Video-MME), and the public LMMs-Eval framework. Code and calibrated configurations will be released upon publication.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://neurips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so \answerNo{} is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://neurips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental setting/details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer) necessary to understand the results?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \textsc{Macer} is training-free and uses fixed backbone-level defaults. Hyperparameters are selected once on a held-out development split disjoint from all reported evaluation sets, then frozen across benchmarks, query types, and retention ratios. No model weights are updated and no optimizer is used.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment statistical significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Mechanism intervention tests in 
    Appendix~\ref{app:null_content} use paired sign tests over 30 paired clips, with exact $p$-values for the direction of mid-layer $\log(v/a)$ shifts (silence: 30/30 pairs, $p=9.3\times10^{-10}$; white noise: 30/30, $p=9.3\times10^{-10}$; mismatched audio: 29/30, $p=2.9\times10^{-8}$). Main benchmark accuracy tables are deterministic evaluations under fixed preprocessing, fixed model weights, greedy decoding, and fixed hyperparameters; for the stochastic Random baseline, the random seed is fixed.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item The authors should answer \answerYes{} if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g., negative error rates).
        \item If error bars are reported in tables or plots, the authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments compute resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Sec.~5.1 specifies the main compute hardware and inference 
    setup, including NVIDIA RTX 6000 Ada 48GB GPUs, greedy decoding, 
    FlashAttention-2, retention ratios, and the FLOPs-accounting protocol. Table~\ref{tab:efficiency_worldsense} reports measured end-to-end latency, prefill time, decode time, and peak memory on a single NVIDIA RTX 6000 Ada GPU. Appendix~\ref{app:efficiency} provides  the FLOPs-ratio accounting used in the main comparison tables. The reported benchmark grid, including main backbone evaluations, baselines, cross-backbone transfer, and ablations, required approximately 500 GPU-hours. Mechanism diagnostics, calibration sweeps, and preliminary runs consumed an additional approximately 1{,}500 GPU-hours.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code of ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The research conforms to the NeurIPS Code of Ethics. It evaluates an inference-time compression method on existing benchmarks and public model backbones, without new human-subject data collection.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer \answerNo, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The work may reduce compute and memory costs for omnimodal inference, making multimodal systems more accessible and efficient. Lower inference cost could also make misuse of deployed multimodal systems cheaper, including large-scale monitoring or surveillance applications; the paper does not release a new model or dataset.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that there is no societal impact of the work performed.
        \item If the authors answer \answerNA{} or \answerNo, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate Deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pre-trained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper does not release a new pretrained model, generated dataset, scraped dataset, or other high-risk asset requiring special release safeguards. The work evaluates an inference-time compression method on existing model backbones and benchmarks.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{}
    \item[] Justification: All existing assets used in this work are cited in
    Sec.~\ref{sec:exp_setup} with their original references. Qwen2.5-Omni-7B/3B are used under the Apache-2.0 license. OmniVinci-9B is used under its publicly released model terms, governed by the NVIDIA OneWay Noncommercial License. The benchmarks are used following their published terms for non-commercial research
    evaluation: AVUTBench and DailyOmni follow their public benchmark releases, WorldSense is released under CC BY-NC-SA 4.0, and Video-MME is released under academic-research-only terms that prohibit commercial use and redistribution. LMMs-Eval is used under the MIT license. We use all assets only for non-commercial research evaluation and do not redistribute benchmark videos, model weights, or derived datasets.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerNA{}{}{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper does not release a new dataset, model checkpoint, benchmark, or other new asset at submission time. It introduces an inference-time compression method and evaluates it on existing model backbones and benchmarks.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset\slash code\slash model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and research with human subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper does not involve crowdsourcing experiments or new research with human subjects. It evaluates an inference-time compression method on existing benchmarks and model backbones.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional review board (IRB) approvals or equivalent for research with human subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper does not involve crowdsourcing or new research with human subjects, and therefore no study participants are recruited and no IRB approval is required. The work evaluates an inference-time compression method on existing benchmarks and model backbones.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\item {\bf Declaration of LLM usage}
    \item[] Question: Does the paper describe the usage of LLMs if it is an important, original, or non-standard component of the core methods in this research? Note that if the LLM is used only for writing, editing, or formatting purposes and does \emph{not} impact the core methodology, scientific rigor, or originality of the research, declaration is not required.
    %this research? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The core method development does not use an additional LLM as an original or non-standard research component, such as for data generation, annotation, evaluation, or experimental decision-making. The OmniLLM backbones used as evaluation targets are described in Sec.~5.1, and any LLM use limited to writing, editing, or formatting does not affect the methodology, scientific rigor, or originality of the research.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the core method development in this research does not involve LLMs as any important, original, or non-standard components.
        \item Please refer to our LLM policy in the NeurIPS handbook for what should or should not be described.
    \end{itemize}

\end{enumerate}

==> old/3_motivation.tex <==
\section{Why Shared Multimodal Attention Is Mis-specified for Compression}
\label{sec:mechanism}

Audio and video are aligned in time, so the most natural way to compress an
interleaved audio--video stream is to score tokens in one common multimodal
space and keep the highest-scoring ones under a shared budget. Existing
compressors differ in how they estimate saliency---shared ranking,
modality-guided pruning, or asymmetric schedules---but they largely inherit
the same default object: token ranking from a shared saliency view
\cite{chen2024fastv,jung2026fastav,tao2025omnizip,ding2026omnisift,li2026dash}.
This view rests on four implicit assumptions about the shared attention 
space: that it is modality-neutral, that its modality preference reflects 
content rather than structure, that it is uniform across depth, and that 
answer-relevant evidence from both modalities emerges at the same layer.

Our diagnostics falsify all four. We show that shared multimodal attention
(i) carries a persistent per-token audio bias that query semantics cannot
overturn (\S\ref{sec:persistent_bias}); (ii) reflects generic content
informativeness rather than query-specific utility, in a graded rather 
than binary fashion (\S\ref{sec:content_responsive}); (iii) decomposes 
into a shallow positional component and a deeper content-driven component 
that a single readout cannot separate (\S\ref{sec:layer_decomposed}); and 
(iv) makes useful audio and video evidence readable at different depths 
(\S\ref{sec:readout_asymmetry}). Together, these findings imply that 
compression decisions grounded in shared attention magnitude are 
mis-specified before any token-ranking rule is applied.

\paragraph{Setup.}
We use paired-query diagnostics on Qwen2.5-Omni-7B over 30 clips. Each 
clip is paired with one \emph{video-essential} query (answerable only 
from visual content) and one \emph{audio-essential} query (answerable 
only from sound). This pairing removes the most obvious confound: that 
the query set itself might be systematically biased toward one modality. 
Unless stated otherwise, videos use the model's default 12-frame setting, 
audio token counts vary naturally with clip duration, and all attention 
statistics are head-aggregated within each layer.

\subsection{A persistent audio bias that queries cannot overturn}
\label{sec:persistent_bias}

If shared multimodal attention were a clean cross-modal saliency space, 
changing the query should suffice to redirect attention toward the 
queried modality. We find that it does not.

Per-token attention mass is systematically higher on audio: $0.000166$ 
per audio token versus $0.000060$ per video token, a $2.8\times$ gap. 
Total attention mass is audio $24.2\%$ versus video $5.2\%$, a $4.6\times$ 
gap. Crucially, this bias is not overturned by the query. Even under 
video-essential queries---where the answer lies strictly in the visual 
stream---audio still receives higher per-token attention than video in 
$87.9\%$ of layer--clip cells; under audio-essential queries, this rises 
to $94.5\%$. A paired-query swap analysis further confirms that query 
semantics produce only a moderate $\sim 1.23\times$ modulation on top of 
this baseline ($p < 0.02$, $26/30$ pairs in the predicted direction), 
which is far too small to invert the baseline preference.

The bias is not a token-packing artifact. A frame-count sweep across 
$\{12, 16, 20\}$ frames shows that the ratio moves monotonically against 
video as more visual tokens are added ($v/a = 0.215, 0.200, 0.179$), so 
the $12$-frame setting is the one most favorable to video, not the one 
that artificially suppresses it. An input-ordering check confirms that 
audio tokens are not packed at the sequence prefix, ruling out a 
front-position sink explanation.

Shared attention magnitude is therefore not a modality-neutral proxy for 
answer relevance. It is already a biased measurement space before any 
compression rule is applied.

\subsection{The bias is content-responsive, not a structural sink}
\label{sec:content_responsive}

A natural next hypothesis is that audio acts as a structural attention 
sink: perhaps the model simply allocates attention to audio tokens 
because they exist, regardless of their content. This would still be 
consistent with the observations above, and it would imply that 
compressing audio is safe essentially by default.

We test this hypothesis with a four-condition null-content intervention 
on $30$ paired clips. We replace the original audio with (i) silence, 
(ii) scale-matched white noise, (iii) \emph{mismatched} audio from an 
unrelated clip (preserving natural acoustic structure but destroying 
semantic alignment with the video), or (iv) original audio as reference. 
If audio attention is structural, all three destructive conditions 
should leave it roughly unchanged. If it is content-responsive, 
attention should collapse when content is destroyed.

The results show a graded collapse. Relative to original audio, the 
median mid-layer $\log(v/a)$ shifts by $+1.80$ under silence, $+1.55$ 
under white noise, and $+0.48$ under mismatched audio. The 
silence-versus-mismatched gap is $\sim 3\times$, and all three effects 
are highly significant ($p = 2.9 \times 10^{-8}$ for mismatched vs.\ 
original under a sign test; $30/30$ monotone for silence/noise vs.\ 
original). The direction is clear: shared attention is not structurally 
allocated to audio. It is evaluating audio content informativeness in a 
graded way---and that is a different quantity from query-specific task 
utility.

This distinction is what makes shared attention a mismatched object for 
compression. A compressor that uses attention magnitude as a cross-modal 
saliency signal will preferentially retain tokens that the model finds 
\emph{generically} informative, not tokens that carry \emph{query-relevant} 
evidence. These two properties correlate, but they are not the same.

\subsection{The bias is layer-decomposed}
\label{sec:layer_decomposed}

The content-responsive bias is not uniform across depth. A distance-matched 
analysis, in which audio and video tokens are compared only when their 
distances to the query token are equalized, reveals two distinct 
components of the bias.

At layer~$10$, equal-distance matching yields a video-to-audio ratio of 
approximately $1.007$: once positional distance is controlled for, the 
audio advantage disappears. The bias at this depth is therefore primarily 
\emph{positional}---audio tokens happen to sit closer to the query in the 
interleaved packing and accumulate recency-driven attention. By 
layer~$14$, the equal-distance ratio drops to $0.484$, and at layer~$19$ 
to $0.412$. A content-driven residual has emerged that persists when 
positional effects are removed.

Two orthogonal controls converge numerically at layer~$14$: the 
distance-matched residual in log ratio is $-0.725$, while the 
null-content mismatched-audio residual from \S\ref{sec:content_responsive} 
is $-0.746$. One experiment controls for position and lets content vary; 
the other controls for content and lets position vary. Their near-identical 
estimates at mid-layer are strong evidence that the content-driven 
component of the audio bias is real and localized to mid-to-late depths.

Figure~\ref{fig:pca} provides a complementary geometric view. In a PCA of 
the query--key interaction space, modality identity is a strong early-layer 
property---audio and video tokens form cleanly separated clusters at 
layers $0$ and $7$---and gradually mixes at deeper layers, consistent with 
the transition from positional to content-driven representation seen in 
the distance-matched analysis.

This layer decomposition has a direct methodological consequence. Any 
compressor that reads saliency from a single shared attention score at a 
single depth conflates positional and content signals. If the goal is to 
preserve answer-critical evidence rather than tokens that happen to sit 
near the query, the decision must be made from representations that 
separate these components rather than entangle them.

\begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth]{figs/obs2.pdf}
    \caption{PCA of the query--key interaction space at layers $0, 7, 13, 
    14, 20, 27$. Audio tokens (blue) and video tokens (red) form sharply 
    separated clusters at early layers and gradually mix at deeper layers. 
    This geometric transition is consistent with the distance-matched 
    analysis in \S\ref{sec:layer_decomposed}: early layers encode 
    modality identity positionally, while deeper layers encode 
    content-driven representations that cut across modality.}
    \label{fig:pca}
\end{figure*}

\subsection{Audio and video expose useful evidence at different depths}
\label{sec:readout_asymmetry}

The final shared-readout assumption is that, even granting the biases 
above, multimodal evidence can still be read out from a single common 
depth. A probe-layer sweep shows this is also not the case. Strong 
operating points are systematically off the shared-depth diagonal: 
useful audio evidence is typically exposed earlier, whereas useful 
video evidence tends to emerge later.

Figure~\ref{fig:readout-sensitivity} summarizes the pattern under a 
fixed allocation configuration across four benchmarks. At the standard 
operating point $\rho = 0.25$, the video axis is consistently steeper 
than the audio axis, with $\Delta_V / \Delta_A$ equal to $8.91\times$ 
on AVUTBench, $1.40\times$ on DailyOmni, $12.50\times$ on Video-MME, 
and $27.00\times$ on WorldSense. The asymmetry is not a universal 
modality law: at the tighter operating point $\rho = 0.10$ on 
AVUTBench, it reverses to $0.76\times$. What remains stable is the 
structural mismatch itself: audio and video do not share the same 
readout profile, so any single common probe depth is systematically 
misaligned with at least one modality.

\begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth]{figs/obs1.pdf}
    \caption{Readout sensitivity and asymmetry across four benchmarks 
    under a fixed allocation configuration. \textbf{(a)} $\Delta_V / 
    \Delta_A$ ratio at two retention ratios; the only cell showing 
    reversal is AVUTBench at $\rho = 0.10$. \textbf{(b)} Per-layer 
    video readout sensitivity, marginalized over $L_a$. All four 
    benchmarks exhibit upward-sloping profiles, indicating a systematic 
    preference for later video readout. \textbf{(c)} Per-layer audio 
    readout sensitivity on the same y-axis scale. Audio profiles 
    remain comparatively flat.}
    \label{fig:readout-sensitivity}
\end{figure*}

Combined with the three preceding findings, this asymmetry closes the 
argument. Shared attention is biased across modalities, its bias 
reflects generic content rather than query-specific utility, it conflates 
positional and content signals across depth, and the optimal readout 
depths for the two modalities do not coincide. A compressor that 
operates on a shared saliency score inherits all four mismatches.


\paragraph{Implication.}
Shared-budget audio--video compression is mis-specified upstream of token ranking. The fix is not to improve the ranking rule within the shared view, but to change the control object.

\textbf{Principle 1.} Shared A/V attention is not a modality-neutral currency, so cross-modal token ranking is the wrong control object.

\textbf{Principle 2.} Query semantics provide only a bounded correction on top of a persistent audio-favoring prior, so budget coordination should be conservative rather than fully dynamic.

\textbf{Principle 3.} The early shared space is distance-driven while the later shared space carries modality preference, so readout must be calibrated robustly rather than chosen by one-cell peak performance.

This is the design adopted by  \method{} 
(\S\ref{sec:method}).

==> old/3_motivation_pre.tex <==
% \section{Observation and Analysis}
% To better understand what an ideal multimodal compression policy should preserve, we construct an \emph{answer-aware oracle proxy} for controlled analysis.
% This oracle is not a deployable policy.
% Instead, it is used to estimate headroom over current methods and to diagnose how useful evidence is distributed across time and modalities on supported multiple-choice benchmarks.

% \subsubsection{Experimental Setup and Definitions}
% We conduct oracle-guided analysis on supported multiple-choice benchmarks, where each example consists of a question $x$, a gold answer option $y^\star$, and synchronized audio-video inputs.
% To make oracle replay comparable to downstream policy evaluation, we partition the input into the same relative temporal bins used in replay and policy construction.

% Let
% \begin{equation}
% \ell(x, A, V; y^\star)=\log p_\theta(y^\star\mid x, A, V)
% \end{equation}
% denote the gold-answer log-probability under the full input, where $A=\{A_t\}_{t=1}^{T}$ and $V=\{V_t\}_{t=1}^{T}$ are the audio and video inputs grouped by relative time bin.
% We measure the contribution of the $t$-th audio or video bin by removing that bin and re-evaluating the model:
% \begin{equation}
% \Delta_t^{(a)}=
% \ell(x, A, V; y^\star)-\ell(x, A_{\setminus t}, V; y^\star),
% \end{equation}
% \begin{equation}
% \Delta_t^{(v)}=
% \ell(x, A, V; y^\star)-\ell(x, A, V_{\setminus t}; y^\star).
% \end{equation}
% A larger value indicates that the removed bin provides stronger support for the correct answer under this oracle proxy.

% Using these oracle scores, we construct oracle-guided replay policies under the same binning and budget protocol as our deployable methods.
% This allows us to compare current policies against an answer-aware upper bound in a controlled setting.

% \subsubsection{Is There Headroom Beyond Deployable Policies?}
% We first ask whether current deployable compression policies are already close to the best answer-aware allocation permitted by the same replay protocol.
% To answer this, we compare them with oracle-guided policies constructed from the gold-answer support scores above.

% We observe that oracle-guided replay consistently outperforms current deployable policies on supported multiple-choice tasks, indicating that existing methods do not yet fully exploit the available multimodal evidence budget.

% \paragraph{Observation 1.}
% \emph{Under the answer-aware oracle proxy, current deployable policies exhibit non-trivial headroom on supported multiple-choice benchmarks.}

% This observation motivates the search for better deployment-time policies, while also clarifying that the oracle should be interpreted as an analysis tool rather than as a realizable inference procedure.

% \subsubsection{Does Modality Relevance Stay Constant Over Time?}
% We next ask whether multimodal relevance can be adequately described by a single fixed audio/video ratio.
% Using the oracle scores $\Delta_t^{(a)}$ and $\Delta_t^{(v)}$, we examine how the relative importance of audio and video changes across temporal bins.

% We find that the preferred modality is not constant over time.
% Some bins are primarily supported by audio evidence, others by video evidence, and some require contributions from both modalities.
% This temporal heterogeneity suggests that a globally fixed cross-modal ratio is too coarse to characterize answer-relevant evidence allocation.

% \paragraph{Observation 2.}
% \emph{Oracle-derived modality relevance is heterogeneous across relative time bins.}

% This observation suggests that effective compression should account for when useful evidence occurs, rather than relying only on a static global modality split.

% \subsubsection{Can Single-Modality Teachers Recover the Joint Oracle?}
% Finally, we ask whether the joint oracle can be explained by a single-modality teacher.
% To do so, we compare oracle-guided policies derived from audio-only scores, video-only scores, and their joint combination.

% We find that single-modality teacher policies do not fully recover the performance of the joint oracle-guided upper bound.
% This indicates that answer-relevant evidence is not fully explained by either modality alone, even when one modality appears dominant in a subset of temporal bins.

% \paragraph{Observation 3.}
% \emph{Single-modality teacher policies do not fully recover the joint oracle upper bound.}

% Taken together, these observations reveal that the challenge in omni-modal compression is not only \emph{how much} budget to keep, but also \emph{where} to place it over time and \emph{how} to coordinate the two modalities.
% Building upon these observations, we next introduce MACER, a deployable policy designed to approximate this structure without access to answer-aware supervision at test time.

% \paragraph{Scope and Limitations.}
% The oracle analysis above is conditioned on gold-answer log-probability, supported multiple-choice evaluation, and a fixed binning-and-replay protocol.
% Accordingly, we treat it as a strong proxy for answer-conditioned importance, rather than as ground-truth causal attribution or a deployable compression strategy.


\section{Observations Motivating Role-Asymmetric Omnimodal Compression}
\label{sec:observations}

To determine what a deployable shared-budget omnimodal compressor must represent, we study three mechanism questions. Rather than asking only whether an answer-aware oracle has headroom over current methods, we ask whether compression error in the omnimodal setting is fully characterized by a single token-ranking problem, or instead arises from several distinct decision objects. In particular, we examine three questions: from which depth each modality most reliably exposes answer-relevant evidence, whether the preferred audio--video allocation is fixed or input-dependent, and whether score-based video retention preserves sufficient temporal support for event-level reasoning. These observations motivate the design of MACER and clarify why a single shared saliency rule is often insufficient under shared audio--video budgets.

% \subsection{Experimental Setup and Diagnostic Protocol}
% \label{subsec:obs_setup}

% We conduct mechanism-oriented analysis on supported multiple-choice benchmarks with synchronized audio--video inputs. Each example consists of a textual query $x$, a gold answer option $y^\star$, and paired multimodal context partitioned into temporal windows. To keep the analysis comparable to deployment-time evaluation, we use the same replay protocol, budget definition, and temporal partitioning as in downstream policy evaluation.

% Our goal in this section is not to introduce a new deployable controller, but to diagnose what structure a deployable compressor must capture. We therefore organize the analysis around three diagnostics. First, we examine layer-dependent modality sensitivity to test whether answer-relevant evidence is exposed at the same depth in audio and video. Second, we analyze how the preferred audio--video allocation varies across inputs and benchmarks under a matched shared budget. Third, we test whether score-driven video retention preserves enough temporal coverage, or instead collapses onto a few local peaks. Together, these diagnostics isolate three distinct failure modes---misplaced readout, suboptimal cross-modal allocation, and temporal-support collapse---that motivate the corresponding design choices in MACER.

\subsection{Do Audio and Video Expose Answer-Relevant Evidence at the Same Depth?}
\label{subsec:obs_readout}

A unified compression rule implicitly assumes that answer-relevant evidence from different modalities can be read out from a comparable representational regime. We first test this assumption by examining modality-specific sensitivity across candidate probe layers. Concretely, we compare how well layer-wise signals from the audio and video branches identify tokens whose removal most affects downstream prediction, and we evaluate which layer choices yield the most reliable operating points under a matched budget protocol.

We observe a stable depth asymmetry between modalities. Audio-relevant evidence is most reliably exposed by relatively shallow probes, whereas video-relevant evidence is more consistently expressed at later layers. This pattern suggests that the two modalities do not share the same readout location, even when they are temporally aligned in the input. A single shared probe therefore conflates two different questions: where audio evidence becomes readable and where video evidence becomes discriminative.

\noindent\textbf{Observation 1.}
\emph{Answer-relevant evidence is read out from different depths in audio and video. Shared-budget omnimodal compression therefore benefits from modality-specific readout, rather than forcing both modalities to compete through a single probe layer or a single shared saliency space.}

This observation motivates the first design choice in MACER: modality-specific evidence readout before any cross-modal competition.

\subsection{Is One Fixed Audio--Video Allocation Sufficient?}
\label{subsec:obs_allocation}

We next ask whether cross-modal competition can be reduced to a single global audio--video ratio. If this were the case, the preferred allocation would remain roughly stable across inputs and temporal regions, and a fixed split would provide an adequate approximation under the shared budget. To test this, we analyze how performance changes under different audio--video shares and how the empirically preferred allocation varies across benchmarks and examples.

We find that the preferred allocation is not constant. Some inputs are primarily constrained by audio evidence, others depend more heavily on video, and many require both modalities but in different proportions. Importantly, this variability is not well described by a single dataset-level average. A fixed share may work reasonably well on one benchmark or one subset of inputs, yet become systematically suboptimal on another. This indicates that allocation is a separate decision object, rather than a byproduct of token ranking within a shared pool.

\noindent\textbf{Observation 2.}
\emph{Optimal audio--video allocation is conditional rather than globally fixed. Effective omnimodal compression must decide not only which tokens to keep within each modality, but also how much capacity each modality should receive under the shared budget.}

This observation motivates the second design choice in MACER: cross-modal coordination should be expressed at the level of budget allocation, rather than by forcing audio and video tokens into a single fused saliency space.

\subsection{Does Score-Based Video Retention Preserve Temporal Support?}
\label{subsec:obs_support}

Even when token saliency is locally informative, video retention faces an additional failure mode that is less severe on the audio side: temporal collapse. A plain global top-$k$ rule can concentrate the retained set on a few sharp score peaks, leaving other time regions unsupported. Such behavior may preserve locally salient frames while still harming event-level reasoning, especially when useful evidence is sparse or distributed over long sequences.

We therefore examine whether high-scoring video retention alone is sufficient to preserve temporal support. Across low- and medium-budget settings, we observe that purely score-driven video selection can become overly localized in time, causing the retained context to miss temporally separated evidence. In contrast, introducing a weak temporal scaffold improves robustness by ensuring that multiple coarse regions remain represented before the remaining capacity is allocated by score. This scaffold does not replace ranking; it prevents ranking from collapsing onto a narrow subset of moments.

\noindent\textbf{Observation 3.}
\emph{Video compression under shared budgets is vulnerable to temporal-support collapse. Preserving a small amount of temporally distributed support matters beyond local token saliency, and it is a distinct requirement from modality-specific readout or cross-modal allocation.}

This observation motivates the third design choice in MACER: applying a weak temporal support prior only on the video branch.

% \subsection{Implication for Method Design}
% \label{subsec:obs_implication}

% Taken together, these observations suggest that shared-budget omnimodal compression is not fully characterized by a single token-ranking problem. Instead, the compressor must resolve three coupled but distinct decisions: where each modality should be read out, how scarce capacity should be split across modalities, and whether retained video evidence remains temporally supported. MACER is designed as a deliberately minimal response to this structure: it performs modality-specific readout, expresses cross-modal interaction only through budget allocation, and applies a weak temporal support prior only on the video branch.

% In this sense, MACER is not introduced as a heavy controller that replaces ranking with a more complicated policy. Rather, it is a minimal factorization of three mechanism-level requirements revealed by the analysis above. The next section shows how these requirements can be instantiated with lightweight, training-free design choices at inference time.

==> old/3_motivation_v2.0.tex <==
% =========================
% Section 3: Motivation
% =========================
\section{Why Shared Readout Is Already Wrong}
\label{sec:motivation}

Audio and video are aligned in time, so the most natural way to compress an
interleaved audio--video stream is to score tokens in one common multimodal
space and keep the highest-scoring ones under a shared budget. Existing
compressors differ in how they estimate saliency---shared ranking,
modality-guided pruning, or asymmetric schedules---but they largely inherit
the same default object: compression is treated primarily as token ranking
from a shared saliency view
\cite{chen2024fastv,jung2026fastav,tao2025omnizip,ding2026omnisift,li2026dash}.
This view is appealing, but it hides a stronger assumption: that the
multimodal space used for compression is already comparable across
modalities, and that answer-relevant evidence from audio and video becomes
usable at roughly the same depth.

Our diagnostics in Fig.~\ref{fig:motivation} suggest that both assumptions
fail. First, shared multimodal attention is not a modality-neutral saliency
space: even on balanced paired queries that symmetrically ask about visual
or auditory content from the same clips, attention remains systematically
biased toward audio on a per-token basis. Second, audio and video do not
share the same readout profile: strong probe configurations are
systematically off the shared-depth diagonal, indicating that useful
evidence becomes readable at different depths in the two modalities.
Together, these results suggest that the main failure begins upstream of
token selection. Under shared-budget compression, the wrong object is not
only the ranking rule; it is the shared readout view itself.

\subsection{Is shared multimodal attention a neutral saliency space?}
\label{sec:attention_bias}

If shared multimodal attention were a clean cross-modal saliency space, then
changing the query should be sufficient to redirect attention toward the
queried modality. To test this directly, we construct balanced paired
queries on the same clips: each clip is paired with one
\emph{video-essential} question, which can only be answered from visual
content, and one \emph{audio-essential} question, which can only be
answered from sound or speech. This design removes the most obvious
alternative explanation for modality imbalance---namely, that the query set
itself may be systematically biased toward audio.

That explanation does not account for the observed pattern
(Fig.~\ref{fig:motivation}, left). Query semantics do shift the audio--video
attention ratio, but only as a moderate correction on top of a persistent
audio prior. Even under \emph{video-essential} queries, audio still
receives higher per-token attention than video in $87.9\%$ of layer--clip
cells; under \emph{audio-essential} queries, this rises to $94.5\%$. The
important point is not that query semantics are irrelevant. The point is
that they are not strong enough to overturn the baseline preference of the
shared attention space.

We therefore do not interpret shared attention magnitude as a clean
cross-modal proxy for answer relevance. It is already a biased measurement
space before any compression rule is applied. A compressor that treats
fused attention as a modality-neutral saliency score is thus built on a
mismatched object from the start.

\subsection{Do audio and video expose useful evidence at the same depth?}
\label{sec:readout}

The next assumption is that, even if multimodal evidence is ranked in a
shared space, it can still be read out from a single common depth. Our
probe-layer study shows that this assumption is too coarse for interleaved
audio--video OmniLLMs (Fig.~\ref{fig:motivation}, right). Strong operating
points are systematically off the shared-depth diagonal: useful audio
evidence is typically exposed earlier, whereas useful video evidence tends
to emerge later.

The key point is not that one particular pair of layers is universally
optimal, nor that audio is intrinsically shallow and video intrinsically
deep in every regime. The fuller retained-ratio sweep shows that the
apparent flatness of the audio axis at standard budgets is conditional on
the operating regime rather than a universal modality law. What remains
stable is the structural mismatch itself: audio and video do not share the
same readout profile, so a single common probe depth is systematically
misaligned with at least one modality.

This finding becomes more consequential in light of the attention
diagnostic above. Once the shared attention space is already known to be
non-neutral, reading both modalities from one common depth compounds the
mismatch: it forces compression to begin from a shared representation that
is biased across modalities and suboptimal for at least one of them. The
failure therefore begins before token ranking. Shared-budget compression in
AV OmniLLMs should not start from a shared readout view.

\paragraph{Implication.}
\emph{Shared-budget audio--video compression is mis-specified upstream of
token ranking. Shared multimodal attention is not a modality-neutral
saliency space, and useful audio and video evidence becomes readable at
different depths. This motivates decoupling evidence readout across
modalities before budgeted token selection.}





% \subsection{Do audio and video expose useful evidence at the same depth?}
% \label{sec:readout}

% Most token-compression methods are written as if compression were primarily a token-ranking problem. In LLMs and VLMs, this usually means pruning from a shared saliency view; recent audio--video compression methods remain close to this perspective even when they introduce modality asymmetry, since the main design object is still token scoring, pruning, or modality-guided selection rather than a separate readout-depth question \cite{chen2024fastv,jung2026fastav,tao2025omnizip,ding2026omnisift,li2026dash}. This is a natural default, but it implicitly assumes that answer-relevant evidence from different modalities becomes usable at roughly the same depth.

% Our probe-layer study shows that this assumption is too coarse for interleaved audio--video OmniLLMs. Strong operating points are systematically off the shared-depth diagonal: useful audio evidence is exposed earlier, whereas useful video evidence tends to emerge later. The key point is not that one particular pair of layers is universally optimal, but that the two modalities do not share the same readout profile.

% The fuller retained-ratio sweep further refines this picture. The apparent flatness of the audio axis at standard budgets is conditional on the operating regime rather than intrinsic to the modality, while the later-readout preference on the video side remains the more stable structural tendency. We therefore do not interpret Obs.~1 as a universal modality law. We interpret it as evidence that the shared-readout assumption is too restrictive for the compression regime of interest.

% \paragraph{Observation}
% \emph{The shared-readout assumption fails in audio--video OmniLLMs. Under shared-budget compression, audio is best read out earlier than video, so a single common probe depth is structurally mismatched to the two modalities.}




\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{figs/obs1.pdf}
\caption{\textbf{Readout sensitivity and asymmetry under MACER's deployment 
allocation.} All sweeps use fixed allocation hyperparameters 
(\texttt{AUDIO\_KEEP\_RATIO}=0.9, \texttt{VIDEO\_FLOOR}=16), matching 
MACER's deployment configuration. 
\textbf{(a)} Asymmetry ratio $\Delta_V/\Delta_A$ across four benchmarks 
at two retention ratios. Video-dominant region ($\Delta_V/\Delta_A > 1$) 
and audio-dominant region ($\Delta_V/\Delta_A < 1$) are shaded. 
AVUTBench at $\rho=0.10$ is the only cell showing reversal.
\textbf{(b)} Per-layer video readout sensitivity, marginalized over 
$L_a$ and centered by per-benchmark task mean. All four benchmarks 
exhibit upward-sloping profiles on the video axis, indicating a 
systematic preference for later video readout.
\textbf{(c)} Per-layer audio readout sensitivity, marginalized over 
$L_v$, on the same y-axis scale. Audio profiles remain comparatively 
flat, producing the $\Delta_V/\Delta_A > 1$ pattern in (a).}
\label{fig:obs1}
\end{figure}




\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{figs/ob2.pdf}
    \caption{
PCA of the query-key interaction space across layers for audio and video tokens.
    Blue points denote audio tokens and red points denote video tokens.
    Early layers show a sharper modality separation, while deeper layers exhibit progressively different overlap and mixing patterns.
    This figure is used as a preliminary diagnostic of how the shared attention space evolves across depth.
    }
    \label{fig:attention_space_layers}
\end{figure*}

% \subsection{Why shared top-$K$ evicts audio}

% A natural extension of video-only compression is to place audio and
% video tokens in one shared pool and retain the top-$K$ tokens under a
% global budget. This removes the need to specify an audio--video split,
% but it assumes that scores from the two modalities are directly
% comparable.

% We find that this assumption fails. Under a shared top-$K$ rule, video
% tokens systematically dominate the retained set, and the effect becomes
% stronger as the budget tightens. On audio-grounded inputs, the retained
% audio fraction collapses and utility drops relative to matched-budget
% per-modality allocation (Table~\ref{tab:allocation_ablation}). This is
% not a hyper-parameter issue: the failure appears before any choice of
% $\alpha$. The problem is not how to tune the split, but whether audio
% and video should compete in one ranking at all.

% \subsection{Why budget allocation, not shared ranking, should coordinate modalities}

% A natural extension of video-only compression is to place audio and
% video tokens in one shared pool and retain the top-$K$ tokens under a
% global budget. This is attractive because it appears to remove the need
% to specify an audio--video split. But it also forces one ranking rule to
% solve two distinct problems at once: how much capacity each modality
% should receive, and which tokens should be kept within that capacity.
% Our diagnostics show that this coupling is the source of failure. Under
% a shared top-$K$ rule, video tokens systematically dominate the retained
% set as the budget tightens, driving the retained audio fraction toward
% zero and hurting utility on audio-grounded inputs relative to
% matched-budget per-modality allocation.

% Separating allocation from ranking reveals a second, stronger
% regularity. Once top-$K$ is applied within each modality, the remaining
% question is no longer whether audio should be protected by a large
% residual share, but how much audio capacity is actually needed before
% returns saturate in practice. Across the six evaluated task--budget
% cells, a low-audio allocation ($\alpha=0.1$, corresponding to realized
% audio retention around $7$--$10\%$ in our setup) yields the lowest
% worst-case empirical regret: its gap to the best observed utility is at
% most $1.25$ points on every cell, within our estimated evaluation noise,
% whereas cap-biased allocation can lose up to $16.63$ points. The point
% is not that every cell shares the exact same optimum. The point is that
% aggressive audio retention is unnecessary as a default: under a matched
% total budget, a small residual audio share already matches the per-cell
% best closely, while freeing the remaining budget for video.

% \paragraph{Observation 2.}
% \emph{Budget split is a first-class decision object in audio--video
% compression. Modalities should coordinate through explicit capacity
% allocation rather than shared token ranking, and the robust default is
% low audio share, not cap-level audio retention.}


% \subsection{Why score-only video retention breaks temporal reachability}
% \label{sec:obs3}

% Once cross-modal competition is removed by capacity allocation (Sec.~\ref{sec:obs2}),
% the video branch reduces to a within-modality selection problem under a fixed budget
% $K_v$. The apparent default is plain global top-$k$ over video saliency scores: it is
% simple, purely score-driven, and matches the ranking view that underlies most prior
% video-LLM compression methods~\citep{chen2024image, jiang2025storm, shao2025holitom}.
% But this view implicitly assumes that answer-relevant evidence on the video branch is
% \emph{locally concentrated}, so that retaining the highest-scoring tokens is sufficient
% to preserve the reasoning signal.

% Our diagnostics show that this assumption fails in a systematic way. Under score-only
% top-$k$, retained video tokens collapse onto a small number of temporally adjacent
% regions, while substantial portions of the timeline receive no retained token at all.
% Crucially, the failure is not visible in token counts---the budget $K_v$ is fully
% spent---but only in the \emph{temporal distribution of answer-conditioned attention
% mass} after compression.

% \paragraph{Reachability diagnostic.} Let $q(j)$ denote the answer-conditioned attention
% weight on video token $j$, obtained by aggregating attention from the first few
% answer-decoding queries over all heads and the calibrated video readout layer
% $\ell_v^\star$. Given a retained subset $\mathcal{S} \subseteq \{1,\dots,n_v\}$ and a
% post-hoc partition of the video timeline into $M$ uniform chunks $\{C_m\}_{m=1}^{M}$,
% we define the \emph{temporal coverage rate}
% \begin{equation}
% \mathrm{TCR}(\mathcal{S}) =
% \frac{1}{M} \left| \Big\{ m :
%     \sum_{j \in \mathcal{S} \cap C_m} q(j)
%     \;\geq\; \theta \cdot \max_{m'}
%     \sum_{j \in \mathcal{S} \cap C_{m'}} q(j)
% \Big\} \right|,
% \label{eq:tcr}
% \end{equation}
% and the \emph{top-1 chunk dominance}
% \begin{equation}
% \mathrm{Dom}(\mathcal{S}) =
% \frac{\max_m \sum_{j \in \mathcal{S} \cap C_m} q(j)}
%      {\sum_m \sum_{j \in \mathcal{S} \cap C_m} q(j)}.
% \label{eq:dom}
% \end{equation}
% $\mathrm{TCR}$ measures how many temporal chunks remain reachable under the retained
% set, while $\mathrm{Dom}$ exposes concentration onto a single chunk. The chunk grid
% $\{C_m\}$ is defined post-hoc and is independent of any chunking used internally by
% MACER, so the metric does not favor scaffold-based methods by construction.

% \paragraph{Result.} Under matched video budgets, score-only global top-$k$ yields a
% substantially lower $\mathrm{TCR}$ and a substantially higher $\mathrm{Dom}$ than the
% full-context reference (Fig.~\ref{fig:reachability}). On video-centric and AV-joint
% benchmarks with long temporal horizons, a non-trivial fraction of timeline chunks
% receive essentially zero retained answer-conditioned mass, even though the budget
% $K_v$ is fully used. A uniform temporal sampling baseline recovers $\mathrm{TCR}$ to
% the full-context level but pays a clear downstream cost, confirming that blind temporal
% spreading is not the right objective either. MACER's weak scaffold, by contrast,
% restores $\mathrm{TCR}$ close to the uniform baseline while preserving downstream
% utility close to score-only top-$k$'s best case---that is, it recovers temporal
% reachability \emph{without} sacrificing saliency.

% \paragraph{Interpretation.} We read this as evidence that temporal support is not a
% diversity heuristic but a \emph{routing constraint} on the video branch. Because
% Qwen2.5-Omni interleaves audio and video tokens along a shared time axis with
% TMRoPE~\citep{xu2025qwen25omni}, answer-conditioned attention on the video branch
% is intrinsically distributed over time, and compression policies that collapse
% retained tokens onto a narrow temporal window sever that routing before the decoder
% can use it. Score-only top-$k$ optimizes a local proxy (per-token saliency) but leaves
% this global reachability property unprotected; a weak support prior is what prevents
% that failure mode.







%backup
% \paragraph{Observation 3.}[Temporal reachability collapse under score-only video retention]
% \label{obs:support}
% Plain score-based top-$k$ on the video branch systematically collapses the temporal
% distribution of retained answer-conditioned attention mass, reducing the number of
% reachable timeline chunks even when the video budget is fully spent. The failure is a
% loss of temporal routing support, not a loss of per-token saliency, and cannot be
% detected from the score ranking alone. A weak temporal coverage prior on the video
% branch is therefore a distinct decision object from readout (Obs.~\ref{obs:readout})
% and allocation (Obs.~\ref{obs:allocation}), completing the decomposition of
% shared-budget omnimodal compression into three non-redundant structural biases.








\subsection{Who guides whom? Let the query decide}


\subsection{What to retain on video? Not just what scores high}







% "OmniZip~\citep{tao2025omnizip} chooses audio as the cross-modal anchor, motivated by their observation that audio tokens receive higher attention in their setting. OmniSIFT~\citep{ding2026omnisift} chooses video as the cross-modal anchor, motivated by their observation that visual structure is the primary carrier of semantic content. Both are defensible under their respective assumptions; their divergence reflects the fact that the right modality to anchor on is ultimately task-dependent. Under shared-budget compression at the inner-LLM stage, this task-dependence can be resolved structurally: query tokens in the LLM prefill are already in dot-product contact with both modalities, so per-modality saliency derived from LLM attention is query-conditioned by construction — the direction of cross-modal importance need not be committed to a priori."






% % ===== motivation figure =====
% \begin{figure*}[t]
%     \centering
%     \begin{subfigure}[t]{0.32\textwidth}
%         \centering
%         \includegraphics[width=\linewidth]{figures/motivation_readout.pdf}
%         \caption{Layer sweep for modality-specific readout.}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[t]{0.32\textwidth}
%         \centering
%         \includegraphics[width=\linewidth]{figures/motivation_allocation.pdf}
%         \caption{Distribution of oracle audio share $\alpha^\star(x;K)$.}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[t]{0.32\textwidth}
%         \centering
%         \includegraphics[width=\linewidth]{figures/motivation_support.pdf}
%         \caption{Temporal-support collapse under global top-$k$ video retention.}
%     \end{subfigure}
%     \caption{
%     Three mechanism diagnostics that reject the null hypothesis of a single shared token-ranking solution for shared-budget omnimodal compression.
%     \textbf{Left:} the best readout depth is systematically earlier for audio than for video, rejecting the shared-readout assumption.
%     \textbf{Middle:} the oracle audio--video budget split varies substantially across inputs, showing that allocation is conditional rather than fixed.
%     \textbf{Right:} score-only video selection collapses temporal support under aggressive retention, while a weak scaffold preserves broader coverage at the same budget.
%     }
%     \label{fig:motivation_overview}
% \end{figure*}



% % ===== mechanism diagnostics table =====
% \begin{table}[t]
% \centering
% \small
% \setlength{\tabcolsep}{4pt}
% \begin{tabular}{lcccc}
% \toprule
% & \multicolumn{2}{c}{Moderate budget} & \multicolumn{2}{c}{Aggressive budget} \\
% \cmidrule(lr){2-3}\cmidrule(lr){4-5}
% Diagnostic & Utility $\uparrow$ & Gain $\uparrow$ & Utility $\uparrow$ & Gain $\uparrow$ \\
% \midrule
% Shared readout (null) & [ ] & -- & [ ] & -- \\
% Modality-specific readout & [ ] & [+ ] & [ ] & [+ ] \\
% \addlinespace[2pt]
% Best fixed split (null) & [ ] & -- & [ ] & -- \\
% Estimated split & [ ] & [+ ] & [ ] & [+ ] \\
% Oracle split & [ ] & [+ ] & [ ] & [+ ] \\
% \addlinespace[2pt]
% Global top-$k$ video (null) & [ ] & -- & [ ] & -- \\
% Scaffolded video retention & [ ] & [+ ] & [ ] & [+ ] \\
% \bottomrule
% \end{tabular}
% \caption{
% Mechanism diagnostics corresponding to the three observations in Sec.~\ref{sec:motivation}. Each block changes only one decision object while matching the total retained-token budget. The gains should remain visible even before combining all three choices into \textsc{MACER}.
% }
% \label{tab:mechanism_diagnostics}
% \end{table}





==> sec/observation.tex <==
\section{observation}

\subsection{Modality-separated ranking vs Unified ranking}


\subsection{}





